LLM-Assisted Code Cleaning For Training Accurate Code Generators

Natural language to code generation is an important application area of LLMs and has received wide attention from the community. The majority of relevant studies have exclusively concentrated on increasing the quantity and functional correctness of training sets while disregarding other stylistic elements of programs. More recently, data quality has garnered a lot of interest and multiple works have showcased its importance for improving performance. In this work, we investigate data quality for code and find that making the code more structured and readable leads to improved code generation performance of the system. We build a novel data-cleaning pipeline that uses these principles to transform existing programs by 1.) renaming variables, 2.) modularizing and decomposing complex code into smaller helper sub-functions, and 3.) inserting natural-language based plans via LLM based transformations. We evaluate our approach on two challenging algorithmic code generation benchmarks and find that fine-tuning CodeLLaMa-7B on our transformed modularized programs improves the performance by up to 30% compared to fine-tuning on the original dataset. Additionally, we demonstrate improved performance from using a smaller amount of higher-quality data, finding that a model fine-tuned on the entire original dataset is outperformed by a model trained on 15% of our cleaned dataset. Even in comparison to closed-source models, our models outperform the much larger AlphaCoder models.

==> figures/introduction/lmdtex1.tex <==
% \begin{figure}
%     \centering
%     \begin{subfigure}{0.48\textwidth}
%     \input{figures/introduction/original_program1}
% \caption{Original program}
%     \end{subfigure}\hfil%
%     \begin{subfigure}{0.48\textwidth}
%     \input{figures/introduction/renamed_program1}
% \caption{Renamed program}
%     \end{subfigure}
%     \begin{subfigure}{0.65\textwidth}
% \input{figures/introduction/modularized_program1}
% \caption{Modularized program}
%     \end{subfigure}
%     \caption{Parallel versions of the same program (from \contests training dataset) generated after the renaming and modularized iterations of our \lmdt approach. \naman{decomposition is perhaps less interesting here since it is mostly about readinput and printoutput -- can find better example where model identifies a more sensible functionality -- however programs become too big. perhaps can fill appendix}}
%     \label{fig:intro:lmdtex1}
% \end{figure}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \begin{mdframed}[leftmargin=0pt,rightmargin=0pt,innerrightmargin=3pt,innerleftmargin=3pt,innertopmargin=0.5pt,innerbottommargin=0.5pt,roundcorner=5pt,backgroundcolor=backcolour]
            \input{figures/introduction/original_program2}
        \end{mdframed}
        \caption{Original program}
    \end{subfigure}\hfil%
    \begin{subfigure}{0.48\textwidth}
        \begin{mdframed}[leftmargin=0pt,rightmargin=0pt,innerrightmargin=3pt,innerleftmargin=3pt,innertopmargin=0.5pt,innerbottommargin=0.5pt,roundcorner=5pt,backgroundcolor=backcolour]
            \input{figures/introduction/renamed_program2}
        \end{mdframed}
        \caption{Renamed program}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
        \begin{mdframed}[leftmargin=0pt,rightmargin=0pt,innerrightmargin=0pt,innerleftmargin=4pt,innertopmargin=0.5pt,innerbottommargin=0.5pt,roundcorner=5pt,backgroundcolor=backcolour]
            \input{figures/introduction/modularized_program2}
        \end{mdframed}
        \caption{Modularized program}
    \end{subfigure}\hfil%
    \begin{subfigure}{0.48\textwidth}
        \begin{mdframed}[leftmargin=0pt,rightmargin=0pt,innerrightmargin=0pt,innerleftmargin=4pt,innertopmargin=0.5pt,innerbottommargin=0.5pt,roundcorner=5pt,backgroundcolor=backcolour]
            \input{figures/introduction/plan_program2}
        \end{mdframed}
        \caption{An explanation for the program}
    \end{subfigure}
    \caption{Parallel versions of the same program (from \contests training dataset) generated after the renaming and modularized iterations of our \lmdt approach.}
    \label{fig:intro:lmdtex1}
\end{figure}


% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}{0.48\textwidth}
%         \begin{mdframed}[leftmargin=0pt,rightmargin=0pt,innerrightmargin=3pt,innerleftmargin=3pt,innertopmargin=0.5pt,innerbottommargin=0.5pt,roundcorner=5pt,backgroundcolor=backcolour]
%             \input{figures/introduction/original_program3}
%         \end{mdframed}
%         \caption{Original program}
%         \label{fig:intro:lmdtex1:orig}
%     \end{subfigure}\hfil%
%     \begin{subfigure}{0.48\textwidth}
%         \begin{mdframed}[leftmargin=0pt,rightmargin=0pt,innerrightmargin=3pt,innerleftmargin=3pt,innertopmargin=0.5pt,innerbottommargin=0.5pt,roundcorner=5pt,backgroundcolor=backcolour]
%             \input{figures/introduction/renamed_program3}
%         \end{mdframed}
%         \caption{Renamed program}
%         \label{fig:intro:lmdtex1:renamed}
%     \end{subfigure}
%     \begin{subfigure}{0.48\textwidth}
%         \begin{mdframed}[leftmargin=0pt,rightmargin=0pt,innerrightmargin=0pt,innerleftmargin=4pt,innertopmargin=0.5pt,innerbottommargin=0.5pt,roundcorner=5pt,backgroundcolor=backcolour]
%             \input{figures/introduction/modularized_program3}
%         \end{mdframed}
%         \caption{Modularized program}
%         \label{fig:intro:lmdtex1:modularized}
%     \end{subfigure}\hfil%
%     \begin{subfigure}{0.48\textwidth}
%         \begin{mdframed}[leftmargin=0pt,rightmargin=0pt,innerrightmargin=0pt,innerleftmargin=4pt,innertopmargin=0.5pt,innerbottommargin=0.5pt,roundcorner=5pt,backgroundcolor=backcolour]
%             \input{figures/introduction/plan_program3}
%         \end{mdframed}
%         \caption{An explanation for the program}
%         \label{fig:intro:lmdtex1:plan}
%     \end{subfigure}
%     \caption{Parallel versions of the same program (from \contests training dataset) generated after the renaming and modularized iterations of our \lmdt approach.}
%     \label{fig:intro:lmdtex1}
% \end{figure}

==> figures/introduction/modularized_program1.tex <==
% \begin{lstlisting}
% import sys

% def read_input():
%     num_vertices, num_edges = map(int, input().split())
%     graph = [[] for _ in range(num_vertices+1)]
%     for _ in range(num_edges):
%         a, b = map(int, input().split())
%         graph[a].append(b)
%         graph[b].append(a)
%     num_operations = int(input())
%     operations = [list(map(int, input().split())) for _ in range(num_operations)]
%     return num_vertices, graph, operations

% def dfs(vertex, distance, color, graph, distances, colors):
%     if distances[vertex] >= distance:
%         return
%     distances[vertex] = distance
%     if colors[vertex] == 0:
%         colors[vertex] = color
%     for neighbor in graph[vertex]:
%         dfs(neighbor, distance-1, color, graph, distances, colors)

% def apply_operations(num_vertices, graph, operations):
%     colors = [0] * (num_vertices+1)
%     distances = [-1] * (num_vertices+1)
%     for vertex, distance, color in operations[::-1]:
%         dfs(vertex, distance, color, graph, distances, colors)
%     return colors[1:]

% def print_output(colors):
%     print("\n".join(map(str, colors)))

% def main():
%     num_vertices, graph, operations = read_input()
%     colors = apply_operations(num_vertices, graph, operations)
%     print_output(colors)

% if __name__ == '__main__':
%     main()        
% \end{lstlisting}
\begin{lstlisting}
def read_input(): (TRUNCATED)

def dfs(vertex, distance, color, graph, distances, colors):
    if distances[vertex] >= distance:
        return
    distances[vertex] = distance
    if colors[vertex] == 0:
        colors[vertex] = color
    for neighbor in graph[vertex]:
        dfs(neighbor, distance-1, color, graph, distances, colors)

def apply_operations(num_vertices, graph, operations):
    colors = [0] * (num_vertices+1)
    distances = [-1] * (num_vertices+1)
    for vertex, distance, color in operations[::-1]:
        dfs(vertex, distance, color, graph, distances, colors)
    return colors[1:]

def print_output(colors):
    print("\n".join(map(str, colors)))

def main():
    num_vertices, graph, operations = read_input()
    colors = apply_operations(num_vertices, graph, operations)
    print_output(colors)

if __name__ == '__main__':
    main()        
\end{lstlisting}

==> figures/introduction/modularized_program2.tex <==
\begin{lstlisting}
def read_input(): ... TRUNCATED

def calculate_distances(graph, distances, k):
  queue = deque()
  queue.append(k)
  distances[k] = 0
  while queue:
    current = queue.popleft()
    for neighbor, neighbor_distance in graph...:
      if distances[neighbor] != -1:
        continue
      distances[neighbor] = distances[current] + ...
      queue.append(neighbor)

def process_queries(graph, distances, num_queries):
  for _ in range(num_queries):
    ...
    print(distances[x] + distances[y])

def main():
  graph, distances, num_queries, k = read_input()
  calculate_distances(graph, distances, k)
  process_queries(graph, distances, num_queries)

main()
\end{lstlisting}

==> figures/introduction/modularized_program3.tex <==
\begin{lstlisting}
def check_if_infinite(num_figures, fig_types):
  index = 0
  while index < num_figures - 1:
    if fig_types[index] + fig_types[index+1] == 5:
      return True
    index += 1
  return False

def calculate_sum_points(num_figures, fig_types):
  index = 0
  sum_points = 0
  while index < num_figures - 1:
    sum_points += fig_types[index] + ...(TRUNCATED)
  return sum_points

def main():
  num_figures = int(input())
  fig_types = list(map(int, input().split()))

  if check_if_infinite(num_figures, fig_types):
    print("Infinite")
  else:
    print("Finite")
    sum_points = calculate_sum_points(num_figures, fig_types)
    print(sum_points)

if __name__ == '__main__':
  main()
\end{lstlisting}

==> figures/introduction/original_program1.tex <==
\begin{lstlisting}
N, M = map(int, input().split())
E = [[] for _ in range(N+1)]
for _ in range(M):
    a, b = map(int, input().split())
    E[a].append(b)
    E[b].append(a)
Q = int(input())
VDC = [list(map(int, input().split())) for _ in range(Q)]
Ans = [0] * (N+1)
D = [-1] * (N+1)

def dfs(v, d, c):
    if D[v] >= d:
        return
    D[v] = d
    if Ans[v]==0:
        Ans[v] = c
    for u in E[v]:
        dfs(u, d-1, c)

for v, d, c in VDC[::-1]:
    dfs(v, d, c)

print("\n".join(map(str, Ans[1:])))
\end{lstlisting}


==> figures/introduction/original_program2.tex <==
\begin{lstlisting}
n=int(input())
G=[[] for i in range(n)]
dist=[-1]*n
for i in range(n-1):
  a,b,c=map(int,input().split())
  G[a-1].append([b-1,c])
  G[b-1].append([a-1,c])

Q,k=map(int,input().split())
k-=1
q=deque()
q.append(k)
dist[k]=0
while q:
  cur=q.popleft()
  for nx,nx_d in G[cur]:
    if dist[nx]!=-1:
      continue
    dist[nx]=dist[cur]+nx_d
    q.append(nx)

for i in range(Q):
  x,y=map(int,input().split())
  x-=1
  y-=1
  print(dist[x]+dist[y])
\end{lstlisting}


==> figures/introduction/original_program3.tex <==
\begin{lstlisting}
n = int(input())
x = list(map(int, input().split()))

i = 0
s = 0
b = True
while i < n-1:
	if x[i]+x[i+1] == 5:
		print("Infinite")
		b = False
		break
	else:
		s += x[i]+x[i+1]
		if i >= 1 and x[i-1]==3 and x[i] == 1 and x[i+1] == 2:
			s-=1
	pass
	i+=1

if b:
	print("Finite")
	print(s)
\end{lstlisting}

==> figures/introduction/plan_program2.tex <==
% \begin{lstlisting}
% 1. `main()`: This is the main function that coordinates the execution of the program. It calls the `read_input()` function to read the input, initializes the `distances` list, and then calls the `calculate_distances()` function to calculate the distances from the vertex `k` to all other vertices in the tree. Finally, it calls the `process_queries()` function to process the queries and print the results.

% 2. `calculate_distances(graph, distances, k)`: This function uses a breadth-first search (BFS) algorithm to calculate the distances from the vertex `k` to all other vertices in the tree. It initializes a queue with the vertex `k` and sets its distance to 0. Then, while the queue is not empty, it dequeues a vertex, updates the distances of its neighbors if they haven't been visited before, and enqueues the neighbors. This process continues until all vertices have been visited and their distances from `k` have been calculated.

% 3. `read_input()`: This function reads the input from the standard input. It first reads the number of vertices `N`, creates an empty graph and initializes a list of distances with -1. Then, it reads `N-1` lines, each containing three integers `a`, `b`, and `c`, which represent an edge between vertices `a` and `b` with length `c`. It adds this edge to the graph. Next, it reads two integers `Q` and `K`, representing the number of queries and the vertex `K` respectively. Finally, it returns the graph, distances, number of queries, and vertex `K`.

% 4. `process_queries(graph, distances, num_queries)`: This function processes the queries by calculating the length of the shortest path from vertex `x` to vertex `y` via vertex `K`, for each query. It reads `num_queries` lines, each containing two integers `x` and `y`. It subtracts 1 from `x` and `y` to convert them to 0-based indexing. Then, it calculates the length of the shortest path by summing the distances of vertices `x` and `y` from vertex `K` and prints the result.
% \end{lstlisting}

\begin{lstlisting}[style=planstyle,basicstyle=\tiny\ttfamily]
1. main()
This is the main function that coordinates the execution of the program. It calls the read_input function to read the input, initializes the distances list, and then calls  calculate_distances function to calculate the distances from the vertex k to all other vertices in the tree. Finally, it calls the process_queries function to process the queries and print the results.


2. read_input() 
... (TRUNCATED)

3. calculate_distances(graph, distances, k)
This function uses a breadth-first search (BFS) algorithm to calculate the distances from the vertex k to all other vertices in the tree. It initializes a queue ... This process continues until all vertices have been visited and their distances from k have been calculated.

4. process_queries(graph, distances, num_queries)
This function processes the queries by calculating ... shortest path by summing the distances of x and y from vertex K and prints the result.
\end{lstlisting}

==> figures/introduction/plan_program3.tex <==

\begin{lstlisting}[style=planstyle,basicstyle=\scriptsize]
1 main()
This is the main function of the program. It first uses the check_if_infinite function to check whether the number of distinct points where figures touch is infinite. If yes, it prints "Infinite". Otherwise, it prints "Finite" and calculates the sum of points where figures touch using `calculate_sum_points function.


2 check_if_infinite(num_figures, fig_types)
This function checks if the number of distinct points where figures touch is infinite. It checks if the sum of adjacent figure types is 5 and returns True


3 calculate_sum_points(...)
This function calculates the sum of points where figures touch. It adds the sum of adjacent figure types to a running total while checking if the square-circle-triangle pattern is found and modifies the sum as appropriate.

\end{lstlisting}


==> figures/introduction/renamed_program1.tex <==
% \begin{lstlisting}
% import sys
% input = sys.stdin.readline
% num_vertices, num_edges = map(int, input().split())
% graph = [[] for _ in range(num_vertices+1)]
% for _ in range(num_edges):
%     a, b = map(int, input().split())
%     graph[a].append(b)
%     graph[b].append(a)
% num_operations = int(input())
% operations = [list(map(int, input().split())) for _ in range(num_operations)]
% colors = [0] * (num_vertices+1)
% distances = [-1] * (num_vertices+1)

% def dfs(vertex, distance, color):
%     if distances[vertex] >= distance:
%         return
%     distances[vertex] = distance
%     if colors[vertex] == 0:
%         colors[vertex] = color
%     for neighbor in graph[vertex]:
%         dfs(neighbor, distance-1, color)

% for vertex, distance, color in operations[::-1]:
%     dfs(vertex, distance, color)

% print("\n".join(map(str, colors[1:])))    
% \end{lstlisting}
\begin{lstlisting}
num_vertices, num_edges = map(int, input().split())
graph = [[] for _ in range(num_vertices+1)]
for _ in range(num_edges):
    a, b = map(int, input().split())
    graph[a].append(b)
    graph[b].append(a)
num_operations = int(input())
operations = [list(map(int, input().split())) for _ in range(num_operations)]
colors = [0] * (num_vertices+1)
distances = [-1] * (num_vertices+1)

def dfs(vertex, distance, color):
    if distances[vertex] >= distance:
        return
    distances[vertex] = distance
    if colors[vertex] == 0:
        colors[vertex] = color
    for neighbor in graph[vertex]:
        dfs(neighbor, distance-1, color)

for vertex, distance, color in operations[::-1]:
    dfs(vertex, distance, color)

print("\n".join(map(str, colors[1:])))    
\end{lstlisting}

==> figures/introduction/renamed_program2.tex <==
\begin{lstlisting}
num_vertices = int(input())
graph = [[] for _ in range(num_vertices)]
distances = [-1] * num_vertices
for _ in range(num_vertices - 1):
  a,b,c = map(int, input().split())
  graph[a-1].append([b-1, c])
  graph[b-1].append([a-1, c])

num_queries, k = map(int, input().split())
k -= 1
queue = deque()
queue.append(k)
distances[k] = 0
while queue:
  current = queue.popleft()
  for neighbor, neighbor_distance in graph...
    if distances[neighbor] != -1:
      continue
    distances[neighbor]=distances[current]+...
    queue.append(neighbor)

for _ in range(num_queries):
  x, y = map(int, input().split())
  x -= 1
  y -= 1
  print(distances[x] + distances[y])    
\end{lstlisting}

==> figures/introduction/renamed_program3.tex <==
\begin{lstlisting}
num_figures = int(input())
fig_types = list(map(int, input().split()))

index = 0
sum_points = 0
is_infinite = True

while index < num_figures - 1:
  if fig_types[index]+fig_types[index+1] == 5:
    print("Infinite")
    is_infinite = False
    break
  else:
    sum_points += fig_types[index] + fig_types[...
    if index >= 1 and fig_types[index-1] == 3 and fig_types[index] == 1 and fig_types...:
      sum_points -= 1
  index += 1

if is_infinite:
  print("Finite")
  print(sum_points)
\end{lstlisting}
